Hitchhiker's Guide to First Year Physics Labs at UCD

This project began as a collection of handouts attempting to provide a slightly more in depth theoretical background to the first year labs performed at University College Dublin. Over time, these handouts were patched together, and this book (if it can be called a book) emerged. The book is intended to complement the University College Dublin first year laboratory manuals, but can also be read independently. The UCD labs span a wide range of subjects, and consequently so do the chapters of this book, beginning with experimental techniques, moving onto classical mechanics, touching on E&M, and ending with a variety of more advanced topics.

==> README <==
Welcome to the README file for the "Hitchhiker's Guide to First Year
Labs" source code. This file is broken down into four parts:

1) License Information
2) Basics
3) Building The Source
4) Modifying The Source

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1) License Information
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

All text and code contained within the source for this book is licensed under
the Creative Commons Attribution 3.0 license. This means that the
source to this book can be freely copied, distributed, and
transmitted. Additionally all source to this book can be modified in
whole or in part, if proper attribution is given to the author.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2) Basics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This book uses LaTeX (http://www.latex-project.org/) as its
typesetting program, specifically through the program "pdflatex". All
figures for the book have been made using Inkscape
(http://www.inkscape.org/), an open source vector graphics
program. All plots for the book have been made using GNU Octave
(http://www.gnu.org/software/octave/) which is a high level numerical
analysis language, similar to MATLAB. The idea behind the software
used to build this book is that it is free and open source.

In top directory of the source there are four directories.

Code -  This directory contains all Octave source code for plots. The
     	Code directory is further split into chapter directories.

Figures - This directory contains the source for all figures used in
	  the book. Currently this includes two types of files: SVG's
	  or scalable vector graphics, and FMP's. The SVG's are
	  readable by Inkscape, while the FMP's are TeX files
	  describing Feynman diagrams using the feynmf language for
	  Feynman diagrams.

Latex - This directory contains all Latex source for the book. Source
      	files are broken down into chapters.

Pdf - Contains all the compiled PDF's including the entire book,
      "book.pdf", and the individual chapters.

For those who are not interested in modifying or compiling the source
for themselves, the Pdf directory will be of the most interest.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 3) Building The Source
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To build the source the following programs and packages must be
installed.

BASH     - version independent (built with version 3.2.39)
PdfLatex - version independent (built with version 3.141592-1.40.3)
MetaPost - version independent (built with version 0.993)
EPSTOPDF - version independent (built with version 2.9.5)
Inkscape - version 0.48 or higher
Octave   - version 3.0.0 (higher versions may work)

If no figures or plots have been added or modified, only BASH and
PdfLatex are required. 

To facilitate simple building of the source, the BASH script
"build.sh" has been written which allows for different build options.

$ ./build.sh book      # builds the entire book
$ ./build.sh lulu      # builds the entire book formatted for Lulu
$ ./build.sh arxiv     # builds a gzipped tar file for the arXiv
$ ./build.sh chapters  # builds the independent chapters
$ ./build.sh <chapter> # builds the specified chapter, e.g. "optics"
$ ./build.sh clean     # removes all generated files
$ ./build.sh cleantop  # cleans only the top directory
$ ./build.sh package   # create a gzipped tar file containing the source

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 3) Modifying The Source
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Perhaps the best way to understand how to modify the source is to go
and explore, but the following guidelines are offered.

When modifying the source to the book, try to remain as consistant
with the current structure as possible. All Octave programs (and any other
programs) should be placed in the approriate chapter subdirectory of
the Code directory, while all figures should be placed in the
appropriate Figures subdirectory. To add a new chapter the appropriate
.tex file must be added in the Latex directory, and new subdirectories
of both Code and Figures must be created.

All Octave functions that produce plots should be written as function
files with the format "functionname(P,varargin)", where the flag P
determines whether the plot is printed to Latex or not. Additionally,
full documentation for each function should be provided. The
"printtex" and "fixlabel" functions should always be used to format
the plot to be included within the Latex document. These two functions
only function when accessed from the top directory of the source.

All Inkscape drawings should be split into two layers, "diagram", and
"text". Additionally, Latex strings should be directly embedded within the
Inkscape drawing. Any text that should not be rendered using the Latex
font of the book should be convereted to a path. Full details on how
the Inkscape document is rendered to pdf and tex is given at
http://wiki.inkscape.org/wiki/index.php/LaTeX

Feynman diagrams are created using a modified version of FeynMP.
http://osksn2.hep.sci.osaka-u.ac.jp/~taku/osx/feynmp.html
The notation on how to draw these diagrams can be a bit tricky, so for
those wanting create new diagrams, explore the online documentation
at, http://www.ctan.org/tex-archive/macros/latex/contrib/feynmf/.

The general idea behind the entire build process is that everything
can be regenerated automatically from within Latex. For this purpose
three special commands have been written.

\includesvg{width}{Chapter}{filename} % includes an SVG from Inkscape
\includeoct{width}{Chapter}{filename} % includes an Octave m-file
\includefmp{width}{Chapter}{filename} % includes a Feynman diagram

Each of these commands takes the source for the image, whether SVG,
m-file, or fmf code, and compares this to the pdf file generated in
the Figures subdirectories. If the source is newer, Latex will
automatically rerun the source through the appropriate program. For these
commands to work however, the proper program names must be set in "book.tex".
Currently the command "octave" is used to invoke Octave, "mpost" to invoke
MetaPost, and "inkscape-0.48pre1" to invoke Inkscape (this one will probably
need to be changed).

